Graph Generation with Variational Recurrent Neural Network

Generating graph structures is a challenging problem due to the diverse representations and complex dependencies among nodes. In this paper, we introduce Graph Variational Recurrent Neural Network (GraphVRNN), a probabilistic autoregressive model for graph generation. Through modeling the latent variables of graph data, GraphVRNN can capture the joint distributions of graph structures and the underlying node attributes. We conduct experiments on the proposed GraphVRNN in both graph structure learning and attribute generation tasks. The evaluation results show that the variational component allows our network to model complicated distributions, as well as generate plausible structures and node attributes.

==> Table/eval_mix_med.tex <==
\begin{table}[t]
\footnotesize
\centering
\setlength{\tabcolsep}{1pt}
\caption{\red{table for mix/med dataset}}
\begin{tabular}{lcccccc}
& \multicolumn{3}{c}{Community-Med (60, $\sim$ 268)} & \multicolumn{3}{c}{Community-Mix (40, $\sim$ 198)}  \\
\toprule
& Degree & Clustering & Orbits & Degree & Clustering & Orbits  \\
\toprule
GraphRNN-RNN &  0.010 & 0.020 & 0.027 & 0.045 & 0.045 & 0.046  \\
\midrule
GraphNRNN-noprior & \textbf{0.010} & 0.026 & 0.029 & 0.043 & 0.051 & 0.047  \\
%GraphNRNN-kld0.5 & 0.012 & 0.025 & 0.028 & 0.038 & 0.047 & 0.039 \\
GraphNRNN-kld1.0 & 0.011 & \textbf{0.019} & \textbf{0.027}  & \textbf{0.036} & \textbf{0.046} & 0.045 \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\label{tlb:mix}
\end{table}
